Stabilizing Performative Feedback Loops with Minimal Model Deployments

When algorithmic predictions inform people's decisions, the models we deploy are performative and actively shape the data we see. This feedback loop between algorithms and their broader environments introduces a challenge in the mechanics of social prediction: If different predictive models induce different distributions, is it possible to efficiently learn a prediction rule that is optimal for the distribution that it induces? Formally, this solution concept is known as performative stability. A core challenge in learning a performatively stable predictor is that, unlike supervised learning where distributions are fixed, the learner must deploy different predictors and observe their induced distributions. The main contribution of our work is a new algorithmic procedure that, in the high-accuracy regime, finds a performatively stable model in nearly the minimum number of model deployments without making any assumptions regarding how predictions shape distributions. In particular, our procedure succeeds at finding a randomized performatively stable predictor using exponentially fewer model deployments than prior approaches. Our second main contribution is a structural result showing how this recent randomized notion of stability achieved by our algorithm can be derandomized into a single predictor satisfying the prior deterministic notion if one is willing to assume that the loss is well-conditioned and that performative effects are weak, as in early work in this area. On a technical level, our results come from building on an underexplored technical connection between performative stability and expected variational inequalities.

==> algo_config.tex <==
\makeatletter
\crefname{algocf}{Algorithm}{Algorithms}
% Fix for line number alignment
%
% (From https://tex.stackexchange.com/questions/476579/how-to-align-line-numbers-horizontally-with-package-algorithm2e)
\patchcmd\algocf@Vline{\vrule}{\vrule \kern-0.4pt}{}{}
\patchcmd\algocf@Vsline{\vrule}{\vrule \kern-0.4pt}{}{}

% Algorithm2e hardcodes a right margin reduction of 1.5em.
% We revert that subtraction almost completely by appending
% to \@algocf@start an addition to \hsize.
\apptocmd{\@algocf@start}{\addtolength{\hsize}{1.4em}}{}{}

% Patch cref's \stepcounter macro to support referencing lines.
%
% (From https://tex.stackexchange.com/questions/103085/algorithm2e-cleveref-problem-with-wrong-reference-to-line-numbers)
\let\cref@old@stepcounter\stepcounter
\def\stepcounter#1{%
    \cref@old@stepcounter{#1}%
    \cref@constructprefix{#1}{\cref@result}%
    \@ifundefined{cref@#1@alias}%
    {\def\@tempa{#1}}%
    {\def\@tempa{\csname cref@#1@alias\endcsname}}%
    \protected@edef\cref@currentlabel{%
        [\@tempa][\arabic{#1}][\cref@result]%
        \csname p@#1\endcsname\csname the#1\endcsname}}

% This function makes an algorithm2e-looking ruled header for an algorithm. This is useful for creating "composite"
% algorithms split into multiple columns.
%
%
\newcounter{algocolumn@line}
\NewDocumentEnvironment {algomulticol} {O{htp!}} {%
    \begin{figure}[#1]%
        \refstepcounter{algocf}%
        \renewcommand\caption[1]{%
            \setlength{\algocf@ruledwidth}{\linewidth}%
            \@algocf@pre@ruled%
            \global\sbox\algocf@capbox{\hskip\AlCapHSkip% .5\algomargin%
                \setlength{\algocf@lcaptionbox}{\hsize}\addtolength{\algocf@lcaptionbox}{-\AlCapHSkip}%
                \parbox[t]{\algocf@lcaptionbox}{\algocf@captiontext{\fnum@algocf}{##1}}
            }%
            \box\algocf@capbox\kern\interspacetitleruled\hrule%
            width\algocf@ruledwidth height\algotitleheightrule depth0pt\kern\interspacealgoruled%
        }%
        \setcounter{algocolumn@line}{0}
        }{%
        \@algocf@post@ruled%
    \end{figure}%
}

\NewDocumentEnvironment {algocolumn} {O{1}m+b} {%
    \scalebox{#1}{%
        \raisebox{6mm}{%
            \begin{minipage}[t]{#2}%
                \RestyleAlgo{plain}%
                \begin{algorithm}[H]%
                    \setcounter{AlgoLine}{\value{algocolumn@line}}% Continue count from previous column
                    #3%
                \end{algorithm}%
            \end{minipage}%
        }%
    }%
}{%
    \setcounter{algocolumn@line}{\value{AlgoLine}}%
}

\makeatother

% Indentation
\SetInd{0.3em}{0.6em}
\NewDocumentCommand \SmallIndentation {} {\SetInd{0.25em}{0.75em}}

% Spacing
\setlength{\interspacetitleruled}{3pt}
\newskip\algoinsideskipamount \algoinsideskipamount=2pt plus 0pt minus 0pt
\def\algoinsideskip{\vspace\algoinsideskipamount}
\SetAlgoInsideSkip{algoinsideskip}
\SetAlCapHSkip{1mm}
\setlength{\algomargin}{5mm}

% Styles
\newcommand{\fnm}[1]{\textsf{#1}}
\newcommand{\kwsty}{\normalfont\bfseries}
\newcommand{\kw}[1]{{\kwsty{}#1}}
\SetAlCapSty{kwsty}
\SetKwSty{kwsty}
\SetFuncSty{fnm}
\SetArgSty{upshape}
\SetFuncArgSty{upshape}
\SetKwComment{Hline}{}{\vspace{-3mm}\textcolor{gray}{\hrule}\vspace{1mm}}
\definecolor{darkgrey}{gray}{0.3}
\definecolor{commentcolor}{gray}{0.5}
\SetKwComment{Comment}{\color{commentcolor}[$\triangleright$\ }{}
\SetCommentSty{}
\SetNlSty{}{\color{black!50}\sffamily}{}

% Keywords
\SetKwProg{XFn}{function}{}{}
\SetKwProg{XSubr}{subroutine}{}{}
\newcommand{\Fn}[1]{\XFn{\normalfont\fnm{#1}}}
\newcommand{\Subr}[1]{\XSubr{\normalfont\fnm{#1}}}
\SetKwFor{ForEach}{for~each}{do}{end}
\crefalias{AlgoLine}{line}%
